Large Language Models Are Not Strong Abstract Reasoners

Large Language Models have shown tremendous performance on a large variety of natural language processing tasks, ranging from text comprehension to common sense reasoning. However, the mechanisms responsible for this success remain opaque, and it is unclear whether LLMs can achieve human-like cognitive capabilities or whether these models are still fundamentally circumscribed. Abstract reasoning is a fundamental task for cognition, consisting of finding and applying a general pattern from few data. Evaluating deep neural architectures on this task could give insight into their potential limitations regarding reasoning and their broad generalisation abilities, yet this is currently an under-explored area. In this paper, we introduce a new benchmark for evaluating language models beyond memorization on abstract reasoning tasks. We perform extensive evaluations of state-of-the-art LLMs, showing that they currently achieve very limited performance in contrast with other natural language tasks, even when applying techniques that have been shown to improve performance on other NLP tasks. We argue that guiding LLM generation to follow causal paths could help improve the generalisation and reasoning abilities of LLMs.

==> experiments/input_dimensionality.tex <==



\subsection{Symbolic Representations}

We generate text and symbolic versions of the ACRE$^T$ and RAVEN$^T$ datasets and study the performance evolution depending on the input format. We focus on the results with RAVEN$^T$-opqa in Table \ref{tab:open_qa_results}, and ACRE$^T$ and RAVEN$^T$-mcqa in Table \ref{tab:mc_qa_results}.

On the ACRE$^T$ dataset, results are better across all models when the input is symbolic, except for GPT-2. This observation is consistent with the idea that the latter does not try to solve the task but only predicts a \textit{plausible} answer, for which an input in natural language is more helpful. 
However, inputs using symbolic data are smaller and may convey only relevant information, while natural language could contain distracting information or biases harmful to task performance.
The same observation can be made concerning RAVEN$^T$-mcqa, except for GPT-4.
In the open-ended version of RAVEN$^T$, models achieve better performance with the natural language representation. Without the answer set available, inductive biases caused by language seem to help performance.



==> experiments/self_refinement_short.tex <==

\subsection{Refinement}

In this section, we investigate various refinement and filtering strategies that have been successful in improving LLM reasoning abilities and see if they can be used to improve abstract reasoning performance. We study two types of strategies: code\textit{-based} and \textit{self-based}. \textit{Code-filtering} is a code-based strategy that consists in generating multiple code responses and filtering out the programs that cannot solve the example cases. \textit{Code-refinement} \citep{DBLP:journals/corr/abs-2309-05660, DBLP:journals/corr/abs-2310-08559} is an iterative process where the model generates a first program. The program is run on the context examples and, if not all answers are correct, the model is prompted to correct its answer based on the output of the interpreter. \textit{Self-filtering} and \textit{self-refinement} \citep{DBLP:journals/corr/abs-2310-08559, DBLP:journals/corr/abs-2303-17651} are similar self-based techniques. They ask the LLM to assess whether the given answer is correct rather than relying on an interpreter. We conduct experiments on BIG-Bench-F and PVR using GPT-4-Turbo (gpt-4-1106-preview). Additional experiments are provided in the appendix.

Table \ref{tab:bench_refinement_short} shows the main results. Overall, the improvements brought by the refinement strategies are limited. The bottleneck in the reasoning is the recognition of the abstract rule linking the context examples. Therefore, the LLM cannot be a good evaluator. This is consistent with the MCQA results observed in Section \ref{sec:mcqa} where the LLMs fail to discriminate the good answers. Unlike self-refinement, self-filtering generates multiple answers independently, not conditioned on the previous iterations. As the LLM performance as a discriminator is above chance, the filtering process can help improving the performance. Code-refinement provides slight improvements in the accuracy for BIG-Bench but decreases it for PVR. The LLMs struggle to accurately exploit the feedback from the interpreter. On BIG-Bench, code-filtering improves the performance the most. The reasons are similar to the self-filtering strategy although the code interpreter is a more rigorous discriminator.

\begin{table}[t]
    \centering
    \caption{Accuracy of refined Large Language Models on BIG-Bench-F and PVR datasets. The best result for each dataset is indicated in \textbf{bold}. Experiments are performed with the latest version of GPT-4 (\textit{gpt-4-1106-preview}). }
    \begin{tabular}{lcc}
        \hline
         & BIG-Bench-F & PVR \\
        \hline
        GPT-4-Turbo-code & 0.280 &\textbf{0.152} \\
        GPT-4-Turbo-code-filtering & \textbf{0.400} & \textbf{0.152} \\
        GPT-4-Turbo-code-refinement & 0.296 & 0.144 \\
        GPT-4-Turbo & 0.268 & 0.000 \\
        GPT-4-Turbo-self-filtering & 0.284 & 0.004 \\
        GPT-4-Turbo-self-refinement & 0.252 & 0.000 \\
        \hline
    \end{tabular}
    \label{tab:bench_refinement_short}
\end{table}
